Explicitising The Implicit Intrepretability of Deep Neural Networks Via Duality

Recent work by Lakshminarayanan and Singh [2020] provided a dual view for fully connected deep neural networks (DNNs) with rectified linear units (ReLU). It was shown that (i) the information in the gates is analytically characterised by a kernel called the neural path kernel (NPK) and (ii) most critical information is learnt in the gates, in that, given the learnt gates, the weights can be retrained from scratch without significant loss in performance. Using the dual view, in this paper, we rethink the conventional interpretations of DNNs thereby explicitsing the implicit interpretability of DNNs. Towards this, we first show new theoretical properties namely rotational invariance and ensemble structure of the NPK in the presence of convolutional layers and skip connections respectively. Our theory leads to two surprising empirical results that challenge conventional wisdom: (i) the weights can be trained even with a constant 1 input, (ii) the gating masks can be shuffled, without any significant loss in performance. These results motivate a novel class of networks which we call deep linearly gated networks (DLGNs). DLGNs using the phenomenon of dual lifting pave way to more direct and simpler interpretation of DNNs as opposed to conventional interpretations. We show via extensive experiments on CIFAR-10 and CIFAR-100 that these DLGNs lead to much better interpretability-accuracy tradeoff.

==> alltables.tex <==
%has 5 blocks of convolutional layers, block 1 has 2 layers with 64 filters,  block 2 has 2 layers with $128$ filters, block 3 has 3 layers with 256 filters, block 4 and 5 have 3 layers of 512 filters, and each block is followed by max-pooling, and the final block is followed by global-average-pooling and then the output layer
\begin{table*}[!h]
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{rcl|c|c|c|c|}\cline{4-7}
 & & &\multicolumn{2}{c|}{VGG (CIFAR-10: 93.6{\tiny{$\pm$0.2}}, CIFAR-100:73.4{\tiny{$\pm$0.3}} )}&\multicolumn{2}{c|}{ResNet(CIFAR-10: 94.0{\tiny{$\pm$0.2}}, CIFAR-100:72.7{\tiny{$\pm$0.2}} )}\\\cline{4-7}
&&&CIFAR-10&CIFAR-100&CIFAR-10&CIFAR-100\\\hline
\multicolumn{1}{|r}{SHALLOW-LIN} &$\stackrel{\text{dual lift}}{\longrightarrow}$&DLGN-SHALLOW&30.6{\tiny{$\pm$0.5}} $\rightarrow$ 84.9{\tiny{$\pm$0.2}} &10.5{\tiny{$\pm$0.2}} $\rightarrow$ 56.3\tiny{$\pm$0.2}&30.6{\tiny{$\pm$0.5}} $\rightarrow$ 80.1\tiny{$\pm$0.2}&10.5{\tiny{$\pm$0.2}} $\rightarrow$49.8\tiny{$\pm$0.9}\\
\multicolumn{1}{|r}{DEEP-LIN} &$\stackrel{\text{dual lift}}{\longrightarrow}$&DLGN&37.8{\tiny{$\pm$0.5}} $\rightarrow$  87.0\tiny{$\pm$0.1}        &15.4{\tiny{$\pm$0.5}} $\rightarrow$ 61.5\tiny{$\pm$0.2} &38.9{\tiny{$\pm$0.1}}   $\rightarrow$    87.9\tiny{$\pm$0.2}    &16.9{\tiny{$\pm$0.1}}$\rightarrow$62.5\tiny{$\pm$0.2}\\
\multicolumn{1}{|r}{SHALLOW-ReLU} &$\stackrel{\text{dual lift}}{\longrightarrow}$&DLGN-SHALLOW& 62.2{\tiny{$\pm$0.2}}$\rightarrow$  84.9{\tiny{$\pm$0.2}}      &36.3{\tiny{$\pm$0.2}}$\rightarrow$ 56.3\tiny{$\pm$0.2} &62.2{\tiny{$\pm$0.2}} $\rightarrow$ 80.1\tiny{$\pm$0.2}       &36.3{\tiny{$\pm$0.2}} $\rightarrow$49.8\tiny{$\pm$0.9} \\
\multicolumn{1}{|r}{DEEP-LIN-MAX} &$\stackrel{\text{dual lift}}{\longrightarrow}$&DLGN-MAX&88.3{\tiny{$\pm$0.1}}$\rightarrow$  92.1\tiny{$\pm$0.1}         &61.8{\tiny{$\pm$0.5}}$\rightarrow$ 69.1\tiny{$\pm$0.1} &84.6{\tiny{$\pm$0.2}}   $\rightarrow$  89.5\tiny{$\pm$0.3}      &57.0{\tiny{$\pm$0.1}}$\rightarrow$66.9\tiny{$\pm$0.1}\\\hline
\end{tabular}
}
\end{table*}


==> analysis.tex <==
\section{Deep Linearly Gated Networks: Complete Disentanglement}
{\centering $\text{DLGN} : x\rightarrow \stackrel{\text{Primal} }{\text{Linear}}\rightarrow \text{Pre-activations}\rightarrow\text{Gates}\stackrel{\text{lifting}}{\rightarrow} \phi_{\Tf}(x) {\rightarrow}\stackrel{\text{Dual} }{\text{Linear}}: \hat{y}(x)=\ip{\phi_{\Tf}(x),v_{\Tv}}$ \par}
 %We continue to be in the DGN setting of characterising learning the weights with fixed gates in the limit of infinite width as in \Cref{sec:fixedgates}. We already saw that this setting is characterised by the NPK. 
%In this section is to present new theoretical insights on prior result and new theoretical results with insights to justify the claim that the learning of the weights given the gates is \emph{disentangled in the path space}. By this, we mean that it is enough to think that the value network is dual linear, i.e., it simply computes/learns the inner product $\hat{y}_{\text{DGN}}=\ip{\phi_{\Tf}(x),v_{\Tv}}$. There are two compelling reasons to adopt the dual view. Reason-(i): In \Cref{sec:gatelearning} we saw that the fixed learnt gates ($79.68\%$) recover almost all the performance of the DNN ($80.32\%$), i.e., dual linearity is not a mere conceptualisation, but is analogous to a linear model in practice as well. In other words, just like one can learn weight vector in a linear model given the features, one can learn the neural path value given the neural path features. Reason-(ii): in the fixed gates infinite width setting, we  already have an interpretation via the NPK.

%In this section is to present new theoretical insights and results to justify the claim that value network is \emph{disentangled in the path space}. By this, we mean that it is enough to think that the value network computes/learns the inner product $\hat{y}_{\text{DGN}}=\ip{\phi_{\Tf}(x),v_{\Tv}}$. There are two compelling reasons to adopt the dual view. Reason-(i): In \Cref{sec:gatelearning} we saw that the fixed learnt gates ($\mathbf{79.68\%}$) recover almost all the performance of the DNN ($\mathbf{80.32\%}$), i.e., dual linearity is not a mere conceptualisation, but is analogous to a linear model in practice as well. In other words, just like one can learn weight vector in a linear model given the features, one can learn the neural path value given the neural path features. Reason-(ii): in the fixed gates infinite width setting, we have an interpretation via the NPK.

The deep linearly gated network (DLGN) has two `mathematically' interpretable linearities, the `primal' and the `dual' linearities. The primal linearity is ensured in via construction and needs no theoretical justification. Once the pre-activations triggers gates, $\phi_{\Tf}(x)$ gets realised in the value network by activating the paths.  Now, the value network itself is `dual' linear, i.e., it simply computes/learns the inner product $\hat{y}(x)=\ip{\phi_{\Tf}(x),v_{\Tv}}$. Gating \emph{lifts} the `primal' linear computations in the feature network to `dual' linear computations in the value network. Dual linearity is characterised by the NPK (for infinite width) which in turn depends on the input and gates, and  the fact that the pre-activations to the gates are primal linear implies complete disentanglement and interpretability. 

Dual linearity is mathematically evident due to the inner product relationship, however, adopting it has the following conceptual issue: it is a commonly held view that `sophisticated features are learnt in the layers', that is, given that the input $x\in\R^{\din}$  is presented to the value network (as in \Cref{fig:dgn}), it could be argued that the GaLUs and linear operations are entangled which in turn enable learning of sophisticated features in the layers. In what follows, we demystify this layer-by-layer view via theory (infinite width case) in \Cref{sec:analysis} , and experiments (on finite width networks) in \Cref{sec:dlgn}, and then study the performance of DLGN in \Cref{sec:dlgn}. The layer-by-layer view is demystified by showing that (i) a constant $\mathbf{1}$ input can be given to the value network, (ii) layer-by-layer structure can be destroyed. The constant $\mathbf{1}$ input is meant to show that if the input is not given to the value network then it is not possible to learn sophisticated structures `from the input' in a layer-by-layer manner.  In terms of the dual linearity, providing a constant $\mathbf{1}$ input has only a minor impact, in that, the neural path feature becomes $\phi(x,p)=1\cdot A(x,p)$, i.e., it still encodes the path activity which is still input dependent. Since $\phi(x)$ depends only on gates, the NPK will depend only on the $\textbf{overlap}$ matrix; results in \Cref{sec:analysis}  captures this in theory. Now, it could be argued that, despite a constant $\mathbf{1}$ input, the gates are still arranged layer-by-layer, due to which, the value network is still able to learn sophisticated structures in its layers. \Cref{sec:analysis} has theory that points out that as long as the \textbf{correlation of the gates} is not lost, the layer-by-layer structure can be destroyed.
% 
%The conceptual issue that stops us from adopting the dual view is the commonly held view that `sophisticated features are learnt in a layer-by-layer' manner. That is, in a DGN, given that the input $x\in\R^{\din}$  is presented to the value network, it could be argued that the GaLUs and linear operations are entangled which in turn enable learning of sophisticated features in the layers. To demystify the layer-by-layer processing viewpoint, in the DGN and DLGN the value network can be provided with a constant $\mathbf{1}$. This is to show that if the input $x\in\R^{\din}$ is not given to the value network in the first place it is not possible to learn sophisticated structures in a layer-by-layer manner. In terms of the dual linearity, providing a constant $\mathbf{1}$ input has only a minor impact, in that, the neural path feature becomes $\phi(x,p)=1\cdot A(x,p)$, i.e., it still encodes the path activity which is still input dependent. Since $\phi(x)$ depends only on gates, the NPK will depend only on the $\textbf{overlap}$ matrix; all the theoretical results in this section will capture the effect. Now, it could be argued that, despite a constant $\mathbf{1}$ input, the gates are still arranged layer-by-layer, due to which, the network is able to still learn sophisticated structures in a layer-by-layer manner. All the results in this section will point out that as long as the \textbf{correlation of the gates} is not lost, the layer-by-layer structure can be destroyed.
\subsection{Dual Linearity: New Insights and New Results}\label{sec:analysis}
%We saw in \Cref{sec:fixedgates} that dual linearity is characterised by the NPK for infinite width case. We now present new insights on \Cref{th:fcprev} by restating it explicitly in terms of the gates in \Cref{th:fc}. We present new results to reveal additional structure of the NPK in the presence of convolutions with global-average-pooling and skip connections in \Cref{th:conv,th:res} respectively and discuss how structure of the NPK helps in demystifying the layer-by-layer view. The motivation for \Cref{th:conv,th:res} that convolutions with pooling and skip connections are quite standard architectural choices and the disentanglement should handle these as well.
%We saw in \Cref{sec:fixedgates} that dual linearity is characterised by the NPK for infinite width case. We now present new insights on \Cref{th:fcprev} by restating it explicitly in terms of the gates in \Cref{th:fc}. Prior work on dual view was for fully connected networks. In this paper, we present new results to reveal additional structure of the NPK in the presence of standard architectural choices namely convolutions with global-average-pooling and skip connections in \Cref{th:conv,th:res} respectively and discuss how structure of the NPK helps in demystifying the layer-by-layer view.
%We saw in \Cref{sec:fixedgates} that dual linearity is characterised by the NPK for infinite width case. We now present new insights on \Cref{th:fcprev} by restating it explicitly in terms of the gates in \Cref{th:fc}. We present new results to reveal additional structure of the NPK in the presence of standard architectural choices namely convolutions with global-average-pooling and skip connections in \Cref{th:conv,th:res} respectively and discuss how  NPK structure helps in demystifying the layer-by-layer view.
We saw in \Cref{sec:fixedgates} that dual linearity is characterised by the NPK for infinite width case. In this section, we: (i) cover standard architectural choices namely convolutions with global-average-pooling and skip connections in \Cref{th:conv,th:res}; the prior result \Cref{th:fcprev} is only for the fully connected case, (ii)  present new insights on \Cref{th:fcprev} by restating it explicitly in terms of the gates in \Cref{th:fc}, and (iii) discuss how the NPK structure helps in demystifying the layer-by-layer view. Note: Results in this section are about the value network and hold for both DGN and DLGN.
%In what follows, we first restate the prior result. While \Cref{th:fc} and Theorem 5.1 in \citep{npk} are mathematically identical, \Cref{th:fc} is written in a manner to capture the fact that the NPK is invariant to permutation of the layers. \Cref{th:conv,th:res} are entirely new and are extensions of the dual view for convolutions with global pooling and skip connections. 


%\subsection{NPK of FC-DNN: Product Kernel }
%\input{cnpkexample}
%\subsection{Neural Path Kernel : Similarity based on active sub-networks}
%\textbf{Remark.} In the case of fully connected networks, $\textbf{overlap}_{\Theta}(i,x,x')$ is equal for all $i\in[\din]$, and hence $\text{NPK}_{\Theta}(x,x')=\ip{x,x'}\cdot\textbf{overlap}_{\Theta}(x,x')$.
%We point out that this statistical decoupling of weights and gates in \Cref{assmp:main} is unrealisable in a DNN with ReLU, however, this assumption can be trivially realised in a DGN. %Further, we are interested only in the `what?' ( and not `how?') question related to the gates in which case this assumptions is not a restriction.
\subsubsection{Fully Connected: Product of LayerWise Base Kernels}
\begin{theorem}
\label{th:fc} Let $G_l(x)\in[0,1]^w$ denote the gates in layer $l\in\{1,\ldots,d-1\}$ for input $x\in\R^{\din}$. Under \Cref{assmp:main}  ($\sigma=\frac{\cscale}{\sqrt{w}}$) as $w\rightarrow \infty $, we have for fully connected DGN/DLGN:
\begin{align*}
\text{NTK}^{\texttt{FC}}(x,x') \rightarrow d \cdot \sigma^{2(d-1)} \cdot \text{NPK}^{\texttt{FC}}(x,x') = d \cdot \cscale^{2(d-1)} \cdot \left(\ip{ x,x'} \cdot \Pi_{l=1}^{d-1} \frac{\ip{G_l(x),G_l(x')}}w\right),
\end{align*}
\end{theorem} 
$\bullet$ \textbf{Product Kernel : Role of Depth and Width.} \Cref{th:fc} is mathematically equivalent to  \Cref{th:fcprev}, which follows from the observation that $\textbf{overlap}(x,x')=\Pi_{l=1}^{(d-1)}\ip{G_l(x),G_l(x')}$. While this observation is very elementary in itself, it is significant at the same time;  \Cref{th:fc} provides the most simplest kernel expression that characterises the information in the gates. From \Cref{th:fc} it is evident that the role of width is \emph{averaging} (due to the division by $w$). Each layer therefore corresponds to a \emph{base kernel} $\frac{\ip{G_l(x),G_l(x')}}w$ which measures the \emph{\textbf{correlation of the gates}}. The role of depth is to provide the product of kernels. To elaborate, the feature network provides the gates $G_l(x)$, and the value network realises the product kernel in \Cref{th:fc} by laying out the GaLUs depth-wise, and connecting them to form a deep network. The depth-wise layout is important: for instance, if we were to concatenate the gating features as $\varphi(x)=(G_l(x),l=1,\ldots,d-1)\in\{0,1\}^{(d-1)w}$, it would have only resulted in the kernel $\ip{\varphi(x),\varphi(x')}=\sum_{l=1}^{d-1}{\ip{G_l(x),G_l(x')}}$, i.e., a \emph{sum  (not product)} of kernels. 

$\bullet$ \textbf{Constant $\mathbf{1}$ Input.} This has a minor impact, in that, the expression on right hand side of \Cref{th:fc} becomes $d \cdot \cscale^{2(d-1)} \cdot \din \cdot \Pi_{l=1}^{d-1} \frac{\ip{G_l(x),G_l(x')}}w$, i.e., the kernel still has information of the gates.

$\bullet$ \textbf{Destroying structure by permuting the layers.}  $\Pi_{l=1}^{d-1} \frac{\ip{G_l(x),G_l(x')}}w$ is permutation invariant, and hence permuting the layers has no effect.


%\textbf{Remark.} Here $\frac{\ip{G_l(x),G_l(x')}}w$ are the \emph{base kernels} measuring the \emph{\textbf{correlation of the gates}}. We show experimentally that the correlation of gates is essentially  `what is learnt in a DNN with ReLUs'.
%and $\Pi_{l=1}^{d-1} \frac{\ip{G_l(x),G_l(x')}}w$ is a product of these base kernels and hence the name `Product of Kernels Theorem'.  The base kernels are essentially measuring which we show via  We now list the roles of the two networks, weights, depth and width.

%\textbf{Feature Network.} The role of this network is to process the input layer-by-layer and produce the $w$-dimensional gating features $G_l(\cdot)$. Each layer comprises of `$w$' ReLUs, and a given ReLU (i.e., gate) is `on' if the input to that layer lies on the positive half-space of hyperplane of given by the incoming weights of that ReLU. Thus the gates of a given layer are based on the angle between the input to that layer and the various hyperplanes given by the weights of that layer. Prior experiments in [\citenum{npk}] and the experiments in this paper show that the feature network, i.e., the gates hold most information, which in turn means that weights of the feature network are key.

%\textbf{Value Network}. The value network implements the product of kernels by laying out the gates as masks depth-wise, and connecting them in the structure of a DNN. Note that depth-wise layout plays an important role here: for instance, if we were to concatenate the gating features as $\varphi(x)=(G_l(x),l=1,\ldots,d-1)\in\{0,1\}^{(d-1)w}$, it would have only resulted in the kernel $\ip{\varphi(x),\varphi(x')}=\sum_{l=1}^{d-1}{\ip{G_l(x),G_l(x')}}$, i.e., a \emph{sum  (not product)} of kernels. Prior experiments in [\citenum{npk}] and the experiments in this paper show that the value network can be reset and re-trained without loss of performance, which in turn means that weights of the value network are not that important.

%\textbf{Note.} The above insights from \Cref{th:main} carry over to the case of DNN with ReLUs by thinking that the roles of value and feature network are performed by a single network.
\subsubsection{Convolution  Global Average Pooling: Rotationally Invariant Kernel}
We consider networks with circular convolution and global average pooling (architecture and notations are in the Appendix). In \Cref{th:conv}, let the circular rotation of vector $x\in\R^{\din}$ by `$r$' co-ordinates be defined as $rot(x,r)(i)=x(i+ r)$, if $i+r \leq \din$ and $rot(x,r)(i)=x(i+ r-\din)$ if $i+r > \din$.  %The architecture and the notations for the network with convolutions is presented in the Appendix. %Using circular convolutions with pooling results in a rotationally invariant kernel \Cref{th:mainconv}.
\begin{comment}
 We extend the dual view to neural network with $\dc$ convolutional layers ($l=1,\ldots,\dc$), followed by a \emph{global-average/max-pooling} layer ($l=\dc+1$) and $\dfc$ ($l=\dc+2,\ldots,\dc+\dfc+1$) fully connected  layers (see Appendix for notation). The convolutional window size is $\wconv<\din$, the number of filters per convolutional layer as well as the width of the fully connected layers is $w$. The main steps are (i) treating pooling layers like gates/masks, (ii) bundling together the paths that share the same path value (due to weight sharing in convolutions) and (iii) re-defining the NPF and NPV for these bundles. The important consequence of weight sharing (due to convolutions and pooling) is that the NPK becomes rotationally invariant resulting in \Cref{th:mainconv}.
\end{comment}
\begin{theorem}\label{th:conv} Under \Cref{assmp:main}, for  a suitable $\bcnn$ (see Appendix for expansion of $\bcnn$):
\begin{align*}
\text{NTK}^{\texttt{CONV}}(x,x')\rightarrow  \frac{\bcnn}{{\din}^2} \cdot \sum_{r=0}^{\din-1} \ip{x,rot(x',r)}_{\textbf{overlap}(\cdot, x,rot(x',r))},\,\, \text{as}\,\,  w\rightarrow\infty\,
\end{align*}
\end{theorem}
$\bullet$ $\sum_{r=0}^{\din-1} \ip{x,rot(x',r)}_{\textbf{overlap}(\cdot, x,rot(x',r))}=\sum_{r=0}^{\din-1}\sum_{i=1}^{\din} x(i) rot(x',r)(i)\textbf{overlap}(i,x,rot(x',r))$, where the inner `$\Sigma$' is the inner product between $x$ and $rot(x',r)$ weighted by $\textbf{overlap}$ and the outer `$\Sigma$' covers all possible rotations, which in addition to the fact that all the variables internal to the network rotate as the input rotates, results in the rotational invariance.  It was observed by \cite{arora2019exact} that networks with global-average-pooling are better than vanilla convolutional networks. The rotational invariance holds for convolutional architectures only in the presence of global-pooling.  So, this result explains why global-average-pooling helps. That said, rotational invariance is not a new observation; it was shown by \cite{li2019enhanced} that  prediction using CNTK-GAP is equivalent to prediction using CNTK without GAP but with full translation data augmentation  (same as rotational invariance) with wrap-around at the boundary (same as circular convolution). However, \Cref{th:conv} is a necessary result, in that, it shows rotational invariance is recovered in the dual view as well. 

$\bullet$ The expression in \Cref{th:conv} becomes $\frac{\bcnn}{{\din}^2} \cdot \sum_{r=0}^{\din-1}\sum_{i=1}^{\din} \textbf{overlap}(i,x,rot(x',r))$  for a \textbf{constant $\mathbf{1}$ input}. The key novel insight is that the rotational invariance is not lost and $\textbf{overlap}$ matrix measures the correlation of the paths which in turn depends on the correlation of the gates.

$\bullet$ \textbf{Destroying structure by permuting the layers} does not destroy the rotational invariance in \Cref{th:conv}. This is because, due to circular convolutions all the internal variables of the network rotate as the input rotates. Permuting the layers only affects the ordering of the layers, and does not affect the fact that the gates rotate if the input rotates, and correlation in the gates is not lost.

\subsubsection{Residual Networks With Skip Connections (ResNet): Ensemble Of Kernels}
We consider a ResNet with `$(b+2)$' blocks and `$b$' skip connections between the blocks. Each block is a fully connected (FC) network of depth `$\dblock$' and width `$w$'. There are $2^b$ many sub-FCNs within this ResNet (see \Cref{def:subfcdnn}).
Note that the blocks being fully connected is for expository purposes, and the result continue to hold for any kind of block.
\input{results}

\begin{definition}\label{def:subfcdnn}[Sub FCNs]
Let $2^{[b]}$ denote the power set of $[b]$ and let $\J\in 2^{[b]}$ denote any subset of $[b]$. Define the`$\J^{th}$' sub-FCN of the ResNet to be the fully connected network obtained by (i) including  $\text{block}_{j},\forall j\in \J$  and (ii) ignoring $\text{block}_{j},\forall j\notin \J$. %(see \Cref{fig:resnet}).
\end{definition}
\begin{theorem}\label{th:res} 
Let $\text{NPK}^{\texttt{FC}}_{\J}$ be the NPK of the $\J^{th}$ sub-FCN, and $\bfc^{\J}$ (see Appendix for expansion of $\bfc^{\J}$) be the associated constant. Under \Cref{assmp:main}, we have:
\begin{align*}
\text{NTK}^{\texttt{RES}}\rightarrow \sum_{\J\in 2^{[b]}}  \bfc^{\J} \text{NPK}^{\texttt{FC}}_{\J}, \,\, \text{as}\,\,  w\rightarrow\infty
\end{align*}
\end{theorem}
%\textbf{Note.} The sub-FC-DNNs we refer to in \Cref{th:mainres} belong to (or are parts of) the feature network from which the gates are obtained. 
$\bullet$ \textbf{Ensemble.} To the best of our knowledge, this is the first theoretical result to show that ResNets have an ensemble structure, where  each kernel in the ensemble, i.e., $\text{NPK}^{\texttt{FC}}_{\J}$ corresponds to one of the $2^b$ sub-architectures (see \Cref{def:subfcdnn}). The ensemble behaviour of ResNet and  presence of $2^b$ architectures was observed by \cite{veit2016residual}, however without any concrete theoretical formalism. 

$\bullet$ Effect of \textbf{constant $\mathbf{1}$ input} is as before for kernels $\text{NPK}^{\texttt{FC}}_{\J}$ and translates to the ensemble $\text{NTK}^{\texttt{RES}}$. 

$\bullet$ \textbf{Destroying structure.} The ResNet inherits the invariances of the block level kernel. In addition, the ensemble structure allows to even remove layers.  \cite{veit2016residual} showed empirically that removing single layers from ResNets at test time does not noticeably affect their performance, and yet removing a layer from architecture such as VGG leads to a dramatic loss in performance. \Cref{th:res} can be seen to provide a theoretical justification for this empirical result. In other words, due to the ensemble structure a ResNet is capable of dealing with failure of components. While failure of component itself does not occur unless one makes them fail purposefully as done in \citep{veit2016residual},  the insight is that even if one or many of the kernels in the ensemble are corrupt and the good ones can compensate.% for them. 


==> bkp.tex <==
\color{blue}
%Training of DGN is explained in \Cref{sec:gatelearning}.

%In the DGN, the external gating signal to the GaLU is derived from the pre-activation input of the corresponding ReLU. 

%The feature network computes the pre-activations in a layer-by-layer manner, the pre-activations from the feature network generate the gates, which are then used to switch

%\subsubsection{Learning Weights With Fixed Gates = Neural Path Kernel}\label{sec:fixedgates}
%During training, a DNN learns both $\phi_{\Theta}(x)$ as well as $v_{\Theta}$ simultaneously, and a finite time characterisation of this learning in finite width DNNs is desirable. However, this is a hard problem. An easier problem is to understand in a DGN, how the weights in the value network are learnt when the gates are fixed in the feature network, i.e., how $\hat{y}_{DGN}(x)=\ip{\phi_{\Tf}(x),v_{\Tv}}$ is learnt by learning $v_{\Tv}$ with fixed $\phi_{\Tf}(x)$. While  $\hat{y}_{DGN}(x)=\ip{\phi_{\Tf}(x),v_{\Tv}}$ is linear in the dual variables, it is still non-linear in the value network weights $\Tv$. However, \cite{npk} showed that the dual linearity is characterised by the NPK in the infinite width regime. We state the assumption followed by Theorem 5.1 in \citep{npk}, wherein, the $\text{NTK}(x,x')=\ip{\nabla_{\Tv}\hat{y}_{\Tdgn_0}(x),\nabla_{\Tv}\hat{y}_{\Tdgn_0}(x') }$ is due to the gradient of $\hat{y}_{\text{DGN}}$ with respect to the value network weights, and the $\text{NPK}(x,x')=\ip{\phi_{\Tf_0}(x),\phi_{\Tf_0}(x')}$ is due to the feature network weights.

%\begin{assumption}\label{assmp:main}
%$\Tv_0\stackrel{\text{i.i.d}}\sim\text{Bernoulli}(\frac12)$ over $\{-{\sigma},+{\sigma}\}$ and statistically independent of $\Tf_0$.
%\end{assumption}
%We point out that this statistical decoupling of weights and gates in \Cref{assmp:main} is unrealisable in a DNN with ReLU, however, this assumption can be trivially realised in a DGN. %Further, we are interested only in the `what?' ( and not `how?') question related to the gates in which case this assumptions is not a restriction.

%\begin{theorem}[Theorem 5.1 in \citep{npk}]
%\label{th:fcprev} Under \Cref{assmp:main} for a fully connected DGN : 
%\begin{align*}
%\text{NTK}^{\texttt{FC}}(x,x')\,\, \stackrel{(a)}\rightarrow\,\, &d \cdot \sigma^{2(d-1)} \cdot \text{NPK}^{\texttt{FC}}(x,x'), \quad\text{as}\,\, w\rightarrow \infty \\
%					     & = d \cdot \sigma^{2(d-1)}\cdot\ip{x,x'}\cdot \textbf{overlap}(x,x')
%\end{align*}
%\end{theorem} 
%\textbf{Remark.} In the fully connected case, $\textbf{overlap}(i,x,x')$ is identical for all $i=1,\ldots,\din$, and hence $\ip{x,x'}_{\textbf{overlap}(\cdot,x,x')}$ in \Cref{lm:npk} becomes $\ip{x,x'}\cdot \textbf{overlap}(x,x')$ in \Cref{th:fcprev}. It follows from NTK theory that an infinite width DGN with fixed gates is equivalent to kernel method with NPK.








\subsubsection{Learning in Gates Key For Finite Width To Be Better Than Infinite Width}\label{sec:gatelearning}
The fixed gates setting is an idealised setting, in that, it does not theoretically capture the learning of the gates, i.e., the neural path features $\phi_{\Theta}(x)$. However, the learning in the gates can be empirically characterised by comparing \textbf{fixed learnt (FL)}  gates coming from a pre-trained DNN and \textbf{fixed random (FR)} gates coming from randomly initialised DNN, and the infinite width NTK.  Using a CNN-GAP and its corresponding DGN, \cite{npk} showed on CIFAR-10 that (see \Cref{fig:dgn} for details on DGN training and the CNN-GAP architecture):

{\centering FR Gates : $\mathbf{67.09\%}\leq $ CNTK-GAP: $\mathbf{77.43\%}\leq $ FL Gates: $\mathbf{79.68\%}\approx $ CNN-GAP: $\mathbf{80.32\%}$\par}

based on which it was concluded that learning in the gates (i.e., neural path features) is crucial for finite width CNN-GAP to outperform the infinite width CNTK-GAP. It was also shown that the DGN can be trained \textbf{standalone} (as shown in \Cref{fig:dgn}) and is only \emph{marginally poor} to the DNN. % this \textbf{explains the open question} in \Cref{sec:ntk}.
%Since the fixed random (FR) gates performed poorly ($67.09\%$) than the best CNTK in \citep{arora2019exact} ($77.43\%$) and the fixed learnt (FL) gates performed better ($79.68\%$) than the best CNTK, 

%Since the fixed learnt gates ($79.68\%$) recover almost all the performance of the DNN ($80.32\%$), it follows that most crucial learning happens in the gates. 
%In other words, dual linearity is not a mere conceptualisation, but is analogous to a linear model in practice as well. That is, just like one can learn weight vector in a linear model given the features, one can learn the neural path value given the neural path features.
 \begin{comment}
\begin{table}
\begin{tabularx}{\columnwidth}{c *{4}{Y}}
\toprule 
CNN-GAP & \multicolumn{3}{c} {CDGN-GAP} \\\cline{2-4}
& Fixed Learnt Gates & Fixed Random Gates & Learnable Gates\\
80.32\% & 79.68\% &67.09\% & 77.12\%\\
\bottomrule
\end{tabularx}
\caption{Data from Table 2 in \citep{npk}.}
\label{tb:cdgn}
\end{table}
\end{comment}
%The information in the gates or the performance of the gates is measured by keeping the gates fixed in the feature network and training the weights of the value network. The key result in \citep{npk} was that the learning in the gates (i.e., the neural path features) improves generalisation, and is the reason behind why finite width DNNs outperforms the infinite width NTK. This result was established empirically by comparing the performance of \textbf{fixed learnt (FL)} gates and that of \textbf{fixed random(FR)} gates and the performance of the NTK in \cite{arora2019exact}. The fixed learnt gates are those that come from a pre-trained feature network (pre-trained using $\hat{y}_\text{f}$) and the fixed random gates are those that come from a randomly initialised feature network. For this purpose, \citep{npk} used a `C4GAP' architecture with $4$ convolutional layers, followed by global-average-pooling (GAP) and a fully connected layer with `softmax' activations. On CIFAR-10, it was observed that the fixed random (FR) gates performed poorly ($68.08\%$) than the NTK in \citep{arora2019exact} ($77.43$) and the fixed learnt (FL) gates performed better ($79.68\%$) than the NTK and within $1\%$ to the C4GAP-DNN ($80.32\%$). Based on this observation it was concluded that (i) gates (encoded as neural path features) are learnt, and (ii) the learning in the gates is the reason for finite width DNN outperforming infinite width NTK. It was also shown that the DGN can be trained standalone, i.e., gates in the feature network and the weights in the value network can be learnt starting from randomised initialisation. The standalone DGN performed only \emph{marginally poor} ($77.12\%$) compared to the DNN ($80.32\%$).

%The test accuracy of C4GAP is approximately $80\%$ on CIFAR-10, and is not state of the art.  However, the main aim here was to compare with the corresponding infinite width NTK whose performance was $77.34\%$ \citep{arora2019exact} for which the C4GAP was sufficient. 



%In a DNN with ReLUs, both the gates (encoded in the neural path features) and the weights (encoded in the neural path value) are learnt by the DNN itself. The DGN setup helps to separate out the learning in the gates (which are learnt in the feature network) and  from the learning in the weights (which are learnt in the value network). Using the DGN, the information in the gates can be measured, by keeping the gates fixed and then training the weights alone. This is equivalent to asking `how good are the neural path features?' and answering it by keeping $\phi_{\Tf}(x)$ fixed and training $v_{\Tv}$ to learn the relation $\hat{y}_{\text{DGN}}(x)=\ip{\phi_{\Tf}(x),v_{\Tv}}$. We now briefly main result in \citep{npk} on fixing gates and learning weights.

%{\centering \emph{{What is the analysis for fixing the gates, i.e., $\phi_{\Tf}(x)$ and learning the weights, i.e., $v_{\Tv}$?}}\par}

%\textbf{Analytical Characterisation of Learning Weights Given Gates.} Recent works \citep{ntk,arora2019exact,cao2019generalization} have connected the training and generalisation of DNNs to kernel methods. An important kernel associated with a DNN is its \emph{neural tangent kernel} (NTK), which, for a pair of input examples $x,x'\in\R^{\din}$, and network weights $\Theta\in\R^{\dnet}$, is given by:
%\begin{align*}
% \text{NTK}(x,x')\quad = \quad \ip{\nabla_{\Theta}\hat{y}(x), \nabla_{\Theta}\hat{y}(x')}
% \end{align*}
%It was shown that, as the width of the DNN goes to infinity, the NTK matrix converges to a limiting deterministic matrix $\text{NTK}_{\infty}$, and training an infinitely wide DNN is equivalent to a kernel method with $\text{NTK}_{\infty}$. Theorem 5.1 in \citep{npk} showed that, when the gates are fixed,  at randomised initialisation, the NTK of an  infinitely wide DGN is equal to (but for a constant factor) the neural path kernel (NPK) which is the Gram matrix of the neural path features. 

%\textbf{Remark:} A previously unnoticed property of the NPK was that it is invariant to layer permutations. Theorem 5.1 in \citep{npk} is not presented here, it is restated in \Cref{th:fc} in which the invariance property is made explicit. 



%\cite{npk} addressed these issues by measuring the performance of the fixed gates. For this, they considered a DGN setup, wherein, the feature network is frozen so as to fix the gates and only the value network is trained. In other words, the gates are fixed the `path features' are fixed, only the `path value' is learnt in the value network. 
%As mention in \Cref{sec:intro}, the key insight in \cite{npk} is that gates play an important role in DNNs with ReLUs. The DGN has external gating, i.e., gates are generated in the feature network and are external to the value network which learns the weights. Note that the neural path features encode the input and the gates, and in the context of DGN, we will be using neural path features as a synonym for the gates. Also the neural path value is learnt in the value network, and in the context of the DGN, we will use neural path value as a synonym for weights. The following question related to learning with external gating lead to the conclusion that gates are key.

%During training, a DNN learns the relation $\hat{y}(x)=\ip{\phi_\Theta(x),v_\Theta}$, i.e., it learns both the neural path features and value. The DGN separately stores $\phi(x)$ and $v$ in the feature and value network respectively and helps in understanding their roles separately.  
%if the feature network weights are fixed, then the gates are fixed and hence the neural path features are fixed as well. 
%Now, training the value network after fixing the gates is linear in the dual variables, and we call this \textbf{dual linearity}. In other words, $\hat{y}_{\text{DGN}}(x)=\ip{\phi_{\Tf}(x),v_{\Tv}}$, is a linear model, where the neural path feature $\phi_{\Tf}(x)\in\R^{\text{total\,paths}}$ is given, and the neural path value $v_{\Tv}\in\R^{\text{total\,paths}}$ needs to be learnt. However, unlike a linear model the various coordinates of $v_{\Tv}$ are not independent variables, but are dependent on each other through the weights (see \Cref{def:npf-npv}). Thus the relation $\hat{y}_{\text{DGN}}(x)=\ip{\phi_{\Tf}(x),v_{\Tv}}$, is non-linear in the weights of the value network. This brings us to the following natural questions, which were answered using the DGN setup:


%The dual view provides the first step in disentangling the linear and the non-linear operations. To elaborate,  it is worthwhile to ask `assuming that we have the \emph{right} neural path features $\phi_{\Tf}(x)$, then can we learn $v_{\Tv}$ separately?'.  This question is worthwhile because, while in each layer of the value network GaLUs and the linear operations are entangled, disentanglement happens in the path variables, i.e., the relation $\hat{y}_{\text{DGN}}(x)=\ip{\phi_{\Tf}(x),v_{\Tv}}$ is linear in the dual variables; we call this \textbf{dual linearity}. Thus, when it comes to the value network alone, we can choose to interpret the computations in a path-by-path manner using dual linearity. This brings us to the next questions of (i) does dual linearity hold in practice?, (ii) are neural path features learnt, and (iii) how to characterise dual linearity analytically, and (iv) can the DGN be an alternative to a DNN? These questions were answered using a DGN setup based on network with $4$ convolutional layers with global average pooling as shown in \Cref{fig:dgn}. 
%\subsection{Experimental Results: Learning in the Gates}


%$\bullet$ \textbf{Fixed Learnt (FL)} gates. Here, the feature network (which is a DNN with ReLU) is \emph{pre-trained} with $\hat{y}_f$ as the output. Then the feature network is frozen and the value network is trained, i.e., in $\hat{y}_{\text{DGN}}(x)=\ip{\phi_{\Tf}(x),v_{\Tv}}$, $\phi_{\Tf}(x)$ is fixed and only $v_{\Tv}$ is learnt. Here, `hard'-gating is used: for pre-activation $q\in\R$, the gating value is $G(q) = \mathbbm{1}_{\{q>0\}}$. It was shown that \emph{most useful information is in the gates/neural path features}, i.e., using a pre-trained DNN as feature network, we can train the value network separately from scratch and match the performance of the pre-trained DNN.  See in \Cref{fig:dgn} the performance of DNN ($80.32$) is close (within $1\%$) to that of the DGN ($79.68$).

%$\bullet$ \textbf{Fixed Random (FR)} gates is similar to the FL gates, expect that, in the `FR gates' the feature network is randomly initialised and kept frozen, and only the value network is trained. Here too, hard gating is used. It was shown that  random gates/neural path features perform significantly poorly than the learnt gates/neural path features. See in \Cref{fig:dgn} the performance of DGN in the FR mode ($68.08$) which is poorer by more than $11\%$ when compared to FL mode ($79.68$).

%\textbf{Message.} Since the random gates performed poorly than the NTK and the learnt gates performed better than the NTK and close to the original DNN itself, it was concluded that (i) gates (encoded as neural path features) are learnt, and (ii) the learning in the gates is the reason for finite width DNN outperforming infinite width NTK. \cite{npk} also showed that the gates and the weights can be learnt simultaneously in a DGN. This is answered by operating the DGN in the \textbf{decoupled learning (DL)} mode, wherein, both the feature and value networks are trained starting from random initialisation. Here, `soft'-gating is used, where, $G(q)=\frac{1}{1+\exp({-\beta\cdot q})}$ ($\beta=$ 4 or 10 are typical choices): this enables gradient to flow via the feature network. It was shown that DGN performs only marginally poorly compared to a DNN. See in \Cref{fig:dgn} the performance of DGN in the DL mode ($77.12$) which is poorer by only around than $3\%$ when compared to DNN ($80.32$). 


%In other words, using pre-trained $\phi_{\Tg}(x)$ we can train the $v_{\Tv}$, in a manner analogous to linear models wherein given the features we can train the weights. 
%\textbf{Key Takeaways.} The dual view gives us an alternate way to look at feature learning. We know that $\phi(x)$s are features using which we can learn $v$s, and that $\phi(x)$s are learnt, and also that the information in the 
%\textbf{DGN Training.} The primary use of the DGN was to measure the information in the gates of a DNN with ReLU. For this, the feature network (which is a DNN with ReLU) is \emph{pre-trained} with $\hat{y}_f$ as the output. Then the feature network is frozen and the value network is trained, i.e., in $\hat{y}_{\text{DGN}}(x)=\ip{\phi_{\Tf}(x),v_{\Tv}}$, $\phi_{\Tf}(x)$ is fixed and only $v_{\Tv}$ is learnt. Here, `hard'-gating is used: for pre-activation $q\in\R$, the gating value is $G(q) = \mathbbm{1}_{\{q>0\}}$. The secondary use of DGN is as an alternative/competetive model (for DNN) that learns  $\hat{y}_{\text{DGN}}(x)=\ip{\phi_{\Tf}(x),v_{\Tv}}$, by separately learning $\Tf$ and $\Tv$ starting from randomised initialisation.Here, `soft'-gating is used, where, $G(q)=\frac{1}{1+\exp({-\beta\cdot q})}$ ($\beta=10$ is a typical choice): this enables gradient to flow via the feature network. 


\begin{comment}

We now discuss the `black box'-ness issue in DNNs and the \emph{neural tangent kernel} based interpretation of DNNs, and the insights from the dual view.


Each layer of a DNN entangles the linear computation with the non-linear activations. The commonly held view  is that such entanglement is the key to success of DNNs, in that, it allows the DNN to learn sophisticated structures in a layer-by-layer manner (we call this the primal view). However, in terms of interpretability, such entanglement has an adverse effect: only the final layer is linear and amenable to a feature/weight interpretation, and neither the feature, i.e., the penultimate layer output, nor the outputs of the intermediate hidden layers are interpretable due to the presence of non-linear activations. 

Recent works [\citep{ntk,arora2019exact,cao2019generalization}] have connected the training and generalisation of DNNs to kernel methods. An important kernel associated with a DNN is its \emph{neural tangent kernel} (NTK), which, for a pair of input examples $x,x'\in\R^{\din}$, and network weights $\Theta\in\R^{\dnet}$, is given by:
\begin{align*}
 \text{NTK}(x,x')\quad = \quad \ip{\nabla_{\Theta}\hat{y}(x), \nabla_{\Theta}\hat{y}(x')}, \quad\text{where}
\end{align*}
$\hat{y}_\Theta(\cdot)\in\R$ is the DNN output. 
It was shown that, as the width of the DNN goes to infinity, the NTK matrix converges to a limiting deterministic matrix $\text{NTK}_{\infty}$, and training an infinitely wide DNN is equivalent to a kernel method with $\text{NTK}_{\infty}$. 

While the NTK provides a kernel interpretation it has the following issues: 

(i) Finite width DNN outperforms its infinite width NTK counterpart \citep{arora2019exact}, that is, the NTK does not fully explain the success of finite width DNNs.

(ii) The NTK is a fixed matrix and hence does not capture representation learning.

(iii) The NTK does not address the issue of entanglement.

We will now discuss the fundamental insights obtained due to the dual view and the DGN setup. 

\textbf{Finite Width vs Infinite Width.} To understand this issue, \cite{npk} measured the performance of fixed gates. For this, they considered a DGN setup, wherein, the feature network is weights are fixed so as to fix the gates and only the value network is trained. In other words, since the gates are fixed, the  neural path features are fixed as well, only the neural path value is learnt in the value network. They showed that the fixed gates from a randomly initialised DNN performed poorly than the NTK and that fixed gates from a pre-trained DNN performed (i) better than the infinite width NTK and (ii) close to the pre-trained DNN itself. This shows that learning in the gates, i.e., neural path features is difference between finite and infinite width networks.

\textbf{Representation Learning.} \citep{npk} showed that in an infinite width fully connected DGN with its gates fixed, the NTK is equal (up to a scalar) to the so called \emph{neural path kernel} (NPK) (equal to the Gram matrix of the neural path features). 
A key difference between the NTK and NPK is that the following: NTK is the kernel corresponding to randomised initialisation, however NPK being the Gram matrix of neural path features is entirely dependent on the input and the gates, wherein, the gates themselves can be either learnt or random. Thus, representation learning is addressed by looking at the NPK corresponding to learnt gates.

\textbf{Entanglement.} Instead of investigating the value network layer-by-layer in which GaLUs and linear operations are entangled, the dual view opens up the option of investigating the value network path-by-path. The path-by-path dual view is more natural because, the value network is \textbf{dual linear}, i.e., it learns a linear function in the neural path features. This gives a subnetwork interpretation:  for each input, only a subset of gates are active, and correspondingly only a subnetwork of the paths are active ( $\phi(x,p)= 0$ if $p$ is inactive). Also, NPK is equal to the \emph{Hadmard} product of the input Gram matrix and a correlation matrix that measures the size of the subnetwork simultaneous active for various pairs of the input examples. In short, the disentanglement happens because the dual view projects the computations onto the path variables.

\end{comment}


\begin{comment}
\begin{definition}[Overlap of active sub-networks]\label{def:overlap} 
The total number of `active' paths for both $x$ and $x'$ that pass through input node $i$ is defined to be:\\
{\centering{\centering{$\textbf{overlap}_{\Theta}(i,x,x') = \Lambda_{\Theta}(i,x,x') \eqdef \left|\{p \colon  A_{\Theta}(x,p)= A_{\Theta}(x',p)=1\}\right|/\din$}}}
\end{definition}
%\subsection{NPK of FC-DNN: Product Kernel }
%\input{cnpkexample}
%\subsection{Neural Path Kernel : Similarity based on active sub-networks}
\begin{lemma}[Neural Path Kernel (NPK)]\label{lm:npk}
Let $D\in\R^{\din}$ be a vector of non-negative entries  and for $u,u'\in\R^{\din}$ , let $\ip{u,u'}_{D}=\sum_{i=1}^{\din}D(i)u(i)u'(i)$. Let $H_{\Theta}(x,x')\eqdef\langle\phi_{\Theta}(x),\phi_{\Theta}(x') \rangle$ be the neural path kernel (NPK). Then  
\begin{align*} 
\text{NPK}_{\Theta}(x,x')= H_{\Theta}(x,x')=\ip{x,x'}_{\Lambda_{\Theta}(\cdot,x,x')} 
\end{align*}
\end{lemma}
\textbf{Remark.} In the case of fully connected networks, $\textbf{overlap}_{\Theta}(i,x,x')$ is equal for all $i\in[\din]$, and hence $\text{NPK}_{\Theta}(x,x')=\ip{x,x'}\cdot\textbf{overlap}_{\Theta}(x,x')$.
\end{comment}


==> concl.tex <==
\section{Conclusion}
Entanglement of the non-linear and the linear operation in each layer of a DNN makes them uninterpretable. This paper proposed a novel DLGN which disentangled the computations in a DNN with ReLUs into two mathematically interpretable linearities, the `primal' linearity from the input to the pre-activations that trigger the gates, and the `dual' linearity in the path space. DLGN recovers more than $83.5\%$ of performance of state-of-the-art DNNs on CIFAR-10 and CIFAR-100. Based on this success of DLGN, the paper  concluded by identifying several interesting future directions.
%asking `Is DLGN a universal spectral approximator?'.

%Entanglement of the non-linear and the linear operation in each layer of a DNN makes them uninterpretable. This paper proposed a novel DLGN which disentangled and rearranged the computations in a DNN with ReLUs in an interpretable manner. 
%The DLGN has two mathematically interpretable linearities, the `primal' linearity from the input to the pre-activations that trigger the gates, and the `dual' linearity in the path space which is characterised by the neural path kernel. 
%It was shown that the disentangled and interpretable computations in a DLGN recover more than $83.5\%$ of performance of state-of-the-art DNNs on CIFAR-10 and CIFAR-100. Based on this success of DLGN, the paper concluded by asking `Is DLGN a universal spectral approximator?'.


==> dlgn.tex <==
\subsection{Numerical Experiments}\label{sec:dlgn}
\Cref{sec:analysis}  presented theoretical results which demystified the layer-by-layer view in value network, in this section we will verify these theoretical results in experiments. We then show that DLGN recovers major part of performance of state-of-the-art DNNs on CIFAR-10 and CIFAR-100.

%$\bullet$ Claim I: \emph{The weight/value network is disentangled in the path space}. 

%$\bullet$ Claim II: \emph{Disentangled computations in a DLGN recovers most performance of DNNs.}

\textbf{Setup Details.} We consider $3$ DNN architectures, C4GAP, VGG-16 and Resnet-110, and their DGN and DLGN counterparts. Here C4GAP is a simple model (achieves about $80\%$ accuracy on CIFAR-10), mainly used to verify the theoretical insights in \Cref{sec:analysis}. VGG-16 and Resnet-110 are chosen for their state-of-the-art performance on CIFAR-10 and CIFAR-100. All models are trained using off-the-shelf optimisers (for more details, see \Cref{sec:expdetails}). The DGN and DLGN are trained from scratch, i.e., both the feature and value network are initialised at random and trained. In DGN and DLGN, we use soft gating (see \Cref{fig:dgn}) so that gradient flows through the feature network and the gates are learnt (we chose $\beta=10$).  In what follows, we use the notation DGN$(\xf,\xv)$ and DLGN$(\xf,\xv)$ where $\xf$ and $\xv$ denote the input to the value and feature networks respectively. For instance, DLGN$(x,x)$ means that both the value and feature network of the DLGN is provided the image as input, and DLGN$(x,\mathbf{1})$ will mean that the feature network is given the image as input and the value network is given a constant $\mathbf{1}$ as input. DGN$(x,x)$ and DGN$(x,\mathbf{1})$ notation works similarly.

\textbf{Disentangling Value Network.} We show that destroying the layer-by-layer structure via permutations and providing a constant $\mathbf{1}$ input do not degrade performance. Since our aim here is not state-of-the-art performance, we use C4GAP with $4$ convolutional layers which achieves only about $80\%$ test accuracy on CIFAR-10, however, enables us to run all the $4!=24$ layer permutations. The C4GAP, DGN and DLGN with layer permutations are shown in \Cref{fig:c4gap}. Once a permutation is chosen, it is fixed during both training and testing. The results in Table I of \Cref{fig:c4gap} show that there is no significant difference in performance between DGN$(x,x)$ vs DGN$(x,\mathbf{1})$, and DLGN$(x,x)$ vs DLGN$(x,\mathbf{1})$, i.e., constant $\mathbf{1}$ input does not hurt. Also, there is no significant difference between the models without permutations and the models with permutations.  These counter intuitive and surprising results are difficult to explain using the commonly held `sophisticated features are learnt layer-by-layer' view. However, neither the permutations or the constant $\mathbf{1}$ input destroys the correlation in the gates, and are not expected to degrade performance as per the insights in \Cref{sec:analysis}. This verifies Claim I.  


\textbf{DLGN Performance.} For this we choose VGG-16 and Resnet-110. The results in Table II of \Cref{fig:c4gap} show that the DLGN recovers more than $83.5\%$ (i.e., $83.78\%$ in the worst case) of the performance of the state-of-the-art DNN. 
While entanglement in the DNNs enable their improved performance,  the `disentangled and interpretable'  computations in the DLGN recovers most part of the performance. 

\subsection{Interesting Future Directions}
Motivated by the success of DLGN, we further break it down into DLGN-\emph{Shallow Features} (DLGN-SF), wherein, the feature network is a collection of shallow single matrix multiplications. We compare a shallow DNN with ReLU called C1GAP against DLGN-SF of C4GAP (see \Cref{fig:shallow}) and VGG-16 (see Appendix). The results are in \Cref{fig:shallow}, based on which we observe the following:

$\bullet$ \textbf{Power of depth in value network and lifting to dual space.} Both C1GAP and C4GAP-DLGN-SF were trained with identical batch size, optimiser and learning rate (chosen to be the best for C1GAP). The performance of C1GAP at $200$ epochs is $\sim10\%$ lower than that of C4GAP-DLGN-SF. After $2000$ epochs of training and ensembling 16 such C1GAPs as C1GAP-\texttt{16-ENS} closes the gap within $\sim 3\%$ on C4GAP-DLGN-SF. Yet, a deeper architecture VGG-16-DLGN-SF is $\sim10\%$ better than C1GAP-\texttt{16-ENS}.  Note that both VGG-16-DLGN-SF and C1GAP-\texttt{16-ENS} have gates for $16$ layers produced in a shallow manner. While in a C1GAP-\texttt{16-ENS}, `16' C1GAPs are ensembled, in VGG-16-DLGN-SF these gates for 16 layers are used as gating signals to turn `on/off' the GaLUs laid depth-wise as 16 layers of the value network, which helps to lift the computations to the dual space. Thus, using the gates to \textbf{lift} (instead of ensembling) the computations to the dual space in the value network is playing a critical role, investigating which is an important future work.%(lifting is caused only if the gates laid out depth-wise as in the value netwrok as opposed to ensemble of 16 models in C1GAP-\texttt{16-ENS}).

$\bullet$ \textbf{Power of depth in feature network.} By comparing CIFAR-100 performance of VGG-16-DLGN-SF in \Cref{fig:shallow} and that of VGG-16-DLGN in \Cref{fig:c4gap}, we see $\sim 6\%$ improvement if we have a deep linear network instead of many shallow linear networks as the feature network. This implies depth helps even if the feature network is entirely linear, investigating which is an important future work. 

$\bullet$ \textbf{DGN vs DLGN} In Table I and II of \Cref{fig:c4gap}, the difference between DGN and DNN is minimal (about $3\%$), however, the difference between DLGN and DNN is significantly large. Thus, it is important to understand the role of the ReLUs in the feature network of DGN. It is interesting to know whether this is simpler than understanding the DNN with ReLUs itself.


$\bullet$ \textbf{Is DLGN a Universal Spectral Approximator?} The value network realises the NPK which in general is an ensemble (assuming skip connections). The NPK is based on the gates whose pre-activations are generated linearly. It is interesting to ask whether the DLGN via its feature network learns the right linear transformations to extract the relevant spectral features (to tigger the gates) and via its value network learns  the ensembling of kernels (based on gates) in a dataset dependent manner.

%To elaborate, any given ReLU in a layer gets triggered if the input to that layer is in the positive half-space corresponding to the hyperplane dictated by the incoming weights of the given ReLU. 
%Consider the domain of image classification. We know that the feature network in a DLGN transforms the input using a sequence of `filter banks', and hence it is possible to use standard tools from `image processing' and `filter banks' theory to understand the meaning of the transformed images in the feature network. Note that if there are non-linearities present then it is not clear as to whether the hidden layer outputs are interpretable as images. 

 %Note that all these questions are related to the feature network, because, we have shown that the role of the gates and the value network is to obtain the gating features and realise the corresponding NPK.



%Recall that in a DLGN, the gating/feature network is a deep linear network without non-linearities, and hence is disentangled by construction. We claimed in \Cref{sec:intro} that the weight/value network is \emph{disentangled in the path space}, for which, as promised we presented theoretical insights in \Cref{sec:analysis}, and now we will provide the supporting experimental evidence. 



%will experimentally compared DNNs with their DGN and DLGN counterparts, to show how the `disentangled and interpretable' computations in a DLGN recover major part of the performance of DNNs. Recall that the gating/


%This also implies that while non-linearity in ReLU causes entanglement (and hence non-interpretability), the major function of the ReLU as gates is to lift the layer-by-layer computations in the gating/feature network to the path-by-path computations in the weight/value network. 
 

%In this section, we turn to the issues of entanglement and `black box'-ness. We start by noting that the performance in the \emph{learnable gates} setting of the DGN show us that the DGN is not only conceptually similar to the DNN, but also empirically approximate to the DNN. In this paper, we modify the DGN to obtain the LGLN. In particular, the LGLN (\Cref{fig:lgln}) is same as the DGN in which (i) the ReLUs in the feature network are replaced with identity activations, and (ii) the input to the value network is $\mathbf{1}$ (see bottom network of LGLN in \Cref{fig:lgln} and the input to the value network of the DGN in \Cref{fig:dgn}). We now discuss how the LGLN disentangles the computations into two linear structures to show that the commonly held view of sophisticated structures are learnt in a layer-by-layer manner is misconceived.  From now on, as it is with the DGN, we will refer to the top part of the LGLN as its feature network and the bottom part as its value network. 



%Continuing with the `learning in gates + learning in the weights given gates' interpretation, using LGLN (\Cref{fig:lgln}), we disentangle both `learning in the gates' as well as `learning in the weights given gates'. 


%We now elaborate on why these changes are needed in the LGLN and how disentangling is achieved.

%$\bullet$ \textbf{Disentangling Feature Network.}  %The gates themselves encode binary information and are triggered by their pre-activations.In a DGN, the transformation from the input to the pre-activation to the gates happens through the hidden layers, in which the linear and non-linear operations are entangled. The hidden layers are not interpretable, and we have to fall back to sophisticated structures being learnt in the hidden layers as an explanation for why it is possible to learn useful pre-activations (as hence useful gates). In LGLN, the non-linear ReLUs are removed, and the transformation in linear, i.e., while the learning of pre-activations happens in a layer-by-layer manner, the learnt structures are no longer sophisticated and are interpretable in terms of standard linear algebra. We will call this \textbf{primal linearity}. Primal linearity is ensured via construction itself and needs no further theoretical justification, and in what follows, we experimentally verify in \Cref{sec:exp} that linearly learnt pre-activations does not degrade performance significantly, when compared to state of the art.

%$\bullet$ \textbf{Disentangling Value Network.} %Note that the value network of the LGLN and that of the DGN are the same, except that in the DGN the value network is given $x\in\R^{\din}$ as the input and in the LGLN it is a constant $\mathbf{1}\in\R^{\din}$ instead.  We show via experiments in \Cref{sec:exp} that destroying the layer-by-layer structure and the constant $\mathbf{1}$ does not degrade performance. These results are counter intuitive, surprising, and more importantly difficult to reconcile with using the `sophisticated features are learnt in a layer-by-layer' explanation. However, we argue that these surprising results can be readily explained using the NPK expression in \Cref{th:fcprev}.  Note that in a DGN, learning the weights with fixed gates amounts to learning a linear model in the dual variables, i.e., learning $\hat{y}_{\text{DGN}}(x)=\ip{\phi_{\Tf}(x), v_{\Tv}}$. We called this \textbf{dual linearity} and in \Cref{sec:prelim} showed that dual linearity has a kernel interpretation in terms of the NPK in \Cref{th:fcprev}. 
%Thus, giving a constant $\mathbf{1}$ input would mean that $\ip{x,x'}=\din$, and the expression on the right reduces to $d \cdot \sigma^{2(d-1)}\cdot \din\cdot \textbf{overlap}(x,x')$. Now a previously unnoticed fact is that $\textbf{overlap}(x,x')$ is invariant to layer permutations, which implies destroying the layer-by-layer structure does not hurt. In short, the main role of the gating non-linearity is to lift the computations from the primal to the dual space. In the dual space, the right way to interpret the computations is path-by-path and the question of sophisticated structures being learnt in the layers is irrelevant.
%However, in terms of the dual variables, the constant $\mathbf{1}$ has the following interpretation: the neural path value is a vector specifying the contribution of each path to the final output and the neural path feature is a vector specifying the path activity (from \Cref{def:npf-npv} $\phi(x,p)=x\cdot A(x,p)$, and since input is $1$, we have $\phi(x,p)=A(x,p)$), i.e., which path to be selected and which one to be left out in the output. The destruction of layers is possible due to the permutation invariance property of the NPK itself which was unnoticed in prior work. 

%In what follows, in \Cref{th:fc}, we first restate Theorem 5.1 in \cite{npk} (i.e., \Cref{th:fcprev}) so as to explicitly capture the permutation invariance. In order to build a  more complete picture, we extend the dual view to cover the cases of convolution with global pooling and skip connections. We then present the aforementioned experimental results in \Cref{sec:exp}.

%What happens when we give $\mathbf{1}$ input to value network?

%What happens when we give permute the gates?

%Interpreting DLGN$(x,\mathbf{1})$

%Interpreting DSLGN$(x,\mathbf{1})$

%Power of Depth Alone


\begin{comment}
\begin{figure}
\centering
\begin{minipage}{1.0\columnwidth}
\centering
\resizebox{0.99\columnwidth}{!}{
\input{fig-c4gap-permute}
}
\resizebox{0.99\columnwidth}{!}{
\input{fig-dlgn-sl-folded}
}
\end{minipage}
\caption{$4$ convolutional layers with GAP}
\label{fig:c4gap}
\end{figure}




\begin{figure}
\centering
\begin{minipage}{1.0\columnwidth}
\centering
\begin{minipage}{0.49\columnwidth}
\resizebox{0.99\columnwidth}{!}{
\input{fig-c4dgngap-permute}
}
\end{minipage}
\begin{minipage}{0.49\columnwidth}
\resizebox{0.99\columnwidth}{!}{
\input{fig-c4lglngap-permute}
}
\end{minipage}
\end{minipage}
\caption{$4$ convolutional layers with GAP}
\label{fig:c4gap}
\end{figure}
\end{comment}

\begin{comment}
\begin{table}[!t]
\centering
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{cccccccc}
\toprule 
Dataset 					& Permute	&CNN-GAP 				&DGN$(x,x)$ 			&DGN$(x,\mathbf{1})$ 	&DLGN$(x,x)$ 			&DLGN$(x,\mathbf{1})$ 	&$\frac{\text{DLGN}(x,\mathbf{1})}{\text{DNN}}$\\\midrule
\multirow{2}{*}{CIFAR10}		& No			&80.5\tiny{$\pm$0.4} 	&77.4\tiny{$\pm$0.3} 	& 77.5\tiny{$\pm$0.2} 	&75.4\tiny{$\pm$0.3} 	&75.4\tiny{$\pm$0.2}		&$93.66$	\\
						& Yes 		&-- 					&77.3\tiny{$\pm$0.5} 	&77.9\tiny{$\pm$0.6}		&75.9\tiny{$\pm$0.5} 	&76.0\tiny{$\pm$0.5}		&$94.40$	\\\midrule
\multirow{2}{*}{CIFAR100}		& No  		&51.8\tiny{$\pm$0.4} 	&47.4\tiny{$\pm$0.2}		&47.3\tiny{$\pm$0.3} 	&47.4\tiny{$\pm$0.1} 	&48.0\tiny{$\pm$0.2}		&$92.66$\\
						& Yes 		& -- 					&48.4\tiny{$\pm$0.8} 	&49.2\tiny{$\pm$0.9} 	&47.5\tiny{$\pm$1.0} 	&48.4\tiny{$\pm$0.9}		&$93.43$\\
\bottomrule
\end{tabular}
}
\caption{\small{All columns (except the last) show the $\%$ test accuracy on CIFAR-10 and CIFAR-100. For each dataset, the top row has results for vanilla models without permutations; the results are averaged over $5$ runs. For each dataset, the bottom row has results of $4!-1=23$ permutations (except the identity) for each model; the results are averaged over the $23$ permutations. The $\%$ of DNN performance recovered by DLGN is in the last column.}} %has the $\%$ of DNN performance that the DLGN recovers.}}
\label{tb:permute}
\end{table}
\end{comment}

\begin{comment}
\begin{table}[!t]
\centering
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{ccccccc}
\toprule 
Dataset 			&C1GAP 				&C1GAP-\texttt{16-ENS}		&C1GAP 				&C1GAP-\texttt{16-ENS}		&C4GAP-DLGN$(x,\mathbf{1})$	&VGG-16-DLGN$(x,\mathbf{1})$\\
\texttt{(epochs)} 		&\texttt{(200)}	 		&\texttt{(200)}				&\texttt{(2000)} 			&\texttt{(2000)}				&\texttt{(50)}					&\texttt{(32)}\\\midrule		
CIFAR-10			&62.2\tiny{$\pm$0.2}		&63.81					&70.0\tiny{$\pm$0.2}		&72.2					&75.1\tiny{$\pm$0.4}				&84.9\tiny{$\pm$0.2}\\ 
CIFAR-100		&36.3\tiny{$\pm$0.2}		&38.23					&42.2\tiny{$\pm$0.3}		&45.47					&47.3\tiny{$\pm$0.6}				&56.3\tiny{$\pm$0.2}\\
\bottomrule
\end{tabular}
}
\caption{\small{}}
\label{tb:shallow}
\end{table}
\end{comment}


\begin{comment}
\begin{table}[!t]
\centering
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{ccccccccc}
\toprule 
Dataset 					& Model 				&DNN 				&DGN$(x,x)$ 			&DGN$(x,\mathbf{1})$ 	&DLGN$(x,x)$ 			&DLGN$(x,\mathbf{1})$ 	&DSLGN$(x,x)$ 		&DSLGN$(x,\mathbf{1})$  \\\midrule
\multirow{2}{*}{CIFAR10}		& C4GAP 				&80.5\tiny{$\pm$0.4} 	&77.4\tiny{$\pm$0.3} 	& 77.5\tiny{$\pm$0.2} 	&75.4\tiny{$\pm$0.3} 	&75.4\tiny{$\pm$0.2}		&74.2\tiny{$\pm$0.2}	 	&73.3\tiny{$\pm$0.2} \\
						& C4GAP-PERMUTE 	&-- 					&77.3\tiny{$\pm$0.5} 	&77.9\tiny{$\pm$0.6}		&75.9\tiny{$\pm$0.5} 	&76.0\tiny{$\pm$0.5}		& -- 					& -- \\\midrule
\multirow{2}{*}{CIFAR100}		& C4GAP 				&51.8\tiny{$\pm$0.4} 	&47.4\tiny{$\pm$0.2}		&47.3\tiny{$\pm$0.3} 	&47.4\tiny{$\pm$0.1} 	&48.0\tiny{$\pm$0.2}		&45.8\tiny{$\pm$0.3}	 	&44.9\tiny{$\pm$0.1}	\\
						& C4GAP-PERMUTE 	& -- 					&48.4\tiny{$\pm$0.8} 	&49.2\tiny{$\pm$0.9} 	&47.5\tiny{$\pm$1.0} 	&48.4\tiny{$\pm$0.9}		& --					& -- \\
\bottomrule
\end{tabular}
}
\caption{Summary of Experiments}
\label{tb:premresults}
\end{table}

\begin{table}[!t]
\centering
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{ccccccccc}
\toprule 
Dataset 					& Model 		&DNN 				&DGN$(x,x)$ 			&DGN$(x,\mathbf{1})$ 	&DLGN$(x,x)$ 			&DLGN$(x,\mathbf{1})$ 	&DSLGN$(x,x)$ 		&DSLGN$(x,\mathbf{1})$  \\\midrule		
\multirow{2}{*}{CIFAR10}		&VGG16-AP 	&93.6\tiny{$\pm$0.2} 	& 93.0\tiny{$\pm$0.1}  	&93.0\tiny{$\pm$0.1}   	&87.0\tiny{$\pm$0.1}		&87.0\tiny{$\pm$0.2}		&84.8\tiny{$\pm$0.3} 	&84.9\tiny{$\pm$0.2} \\
						&ResNet110 	&94.0\tiny{$\pm$0.2} 	& 93.3\tiny{$\pm$0.2} 	&93.2\tiny{$\pm$0.1} 	&87.9\tiny{$\pm$0.2}   	&87.8\tiny{$\pm$0.1} 	&72.4{$\pm$13.8} 		&71.2{$\pm$17.3}  \\\midrule
\multirow{2}{*}{CIFAR100}		&VGG16-AP 	&73.4\tiny{$\pm$0.3}  	&70.3\tiny{$\pm$0.1} 	&70.5\tiny{$\pm$0.2} 	&61.5\tiny{$\pm$0.2}		&61.5\tiny{$\pm$0.1}		&56.4\tiny{$\pm$0.4} 	&56.3\tiny{$\pm$0.2}\\
						&ResNet110 	&72.7\tiny{$\pm$0.2}		&70.8\tiny{$\pm$0.2} 	&70.8\tiny{$\pm$0.4}		&62.3\tiny{$\pm$0.2} 	&62.7\tiny{$\pm$0.3} 	&49.8{$\pm$0.9}		&41.5{$\pm$15.5}  \\
\bottomrule
\end{tabular}
}
\caption{Summary of Experiments}
\label{tb:expresults}
\end{table}
\end{comment}





\begin{comment}
\subsection{Open Question: Upstream training with random labels}\label{sec:exp2}
In this section, we add more evidence in favour of why the dual view is a useful when it comes to disentangling and understanding the inner workings of DNNs with ReLUs. For this, we turn to the study of \cite{randlabel} who studied both positive and negative effects on downstream training performance due to upstream training with random labels. However, the following question on test performance is open: \emph{When trained with random labels upstream followed by true labels downstream, the test performance of a DNN with ReLUs degrades, Why?}

\textbf{Answer Using Dual View}. Let us denote training by true labels by subscript $\text{T}$ and training by random labels first followed by true labels by subscript RT. In what follows, we also drop $\Theta$ from the notation. When trained with true labels, the DNN learns the relation $\hat{y}(x)=\ip{\phi_{\text{T}}(x),v_{\text{T}}}$. The scenario in the open question corresponds to learning  $\hat{y}(x)=\ip{\phi_{\text{RT}}(x),v_{\text{RT}}}$. In order to disentangle the effect of the random labels on the gates and the weights separately, we consider the following two scenarios: (i) learning $\hat{y}(x)=\ip{\phi_{\text{RT}}(x),v_{\text{T}}}$; this can be achieved using the DGN setup by pre-training the feature network first with random labels followed by true labels, and then training the value network with true labels. (ii) learning $\hat{y}(x)=\ip{\phi_{\text{T}}(x),v_{\text{RT}}}$; this can be achieved using the DGN setup by pre-training the feature network with true labels, and then training the value network first with random labels followed by true labels.
\begin{table}[!t]
\centering
%\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{cccc}
\toprule 
$\hat{y}(x)=\ip{\phi_{\text{T}}(x),v_{\text{T}}}$ 	&$\hat{y}(x)=\ip{\phi_{\text{T}}(x),v_{\text{RT}}}$ 	&$\hat{y}(x)=\ip{\phi_{\text{RT}}(x),v_{\text{RT}}}$ 	&$\hat{y}(x)=\ip{\phi_{\text{RT}}(x),v_{\text{T}}}$ 	\\\midrule
80.3\tiny{$\pm$0.2}						&78.2\tiny{$\pm$0.3}							&68.5\tiny{$\pm$0.3}							&69.5\tiny{$\pm$0.2}								\\
\bottomrule
\end{tabular}
%}
\caption{\small{Random labels affect the gates. In column $2$ the random labels were corrupted by $100\%$. In columns $3$ and $4$ the random labels were corrupted by $75\%$, because we could not train the DNN with $100\%$ corrupt labels.}}
\label{tb:randlabel}
\end{table}

We chose the $4$-layer CNN-GAP and and its corresponding DGN to obtain the results in \Cref{tb:randlabel}. It is evident from column $2$ that if the gates, i.e., the neural path features are \emph{clean}, training the weights, i.e., the neural path value with random labels first followed by true labels degrades test performance only by $3\%$. Also, it is evident from column $4$ that if the gates, i.e., the neural path features are \emph{corrupt}, training the weights, i.e., the neural path values with true labels still have poor performance by about $11.5\%$. Based on these, we conclude that, \emph{degradation in the test performance due to upstream training with random labels is  because the gates, i..e, neural path features degrade.}
\end{comment}
%& C4GAP 		& 51.8 \tiny{$\pm$0.4} 	& DGN$(x,x)$ 	& DGN$(x,\mathbf{1})$ 	&  DLGN$(x,x)$ 	& DLGN$(x,\mathbf{1})$ & DSLGN$(x,x)$ 	& DSLGN$(x,\mathbf{1})$\\




%We now present additional theoretical and experimental insights on dual linearity that show that the once the gates are given the learning in the weights is best understood by a path-by-path view and the layer-by-layer view is not relevant.



%Given a DNN, there are two corresponding networks, the LGLN  in \Cref{sec:intro} and the DGN in \Cref{sec:prelim}. The LGLN can be obtained from the DGN by,

%(i) replacing all the ReLU activations in the feature network 

%The DGN performs only marginally poor compared to the DNN, and by successfully addressing the `black box'-ness issue in a DGN we will have both performance and interpretability. We now propose our novel \texttt{DGN-NO-ACT}  which disentangles the computations into (i) primal linear layer-by-layer computation, (ii) dual linear path-by-path computation and (iii) gating non-linearity which \emph{lifts} the computations from the primal to the dual. \texttt{DGN-NO-ACT} (right diagram in \Cref{fig:dgn}) is obtained by making a novel modification to the DGN (left diagram in \Cref{fig:dgn}) as follows:

%1. We replace the ReLUs in the feature network with \emph{identity} maps, i.e., $I(q) = q$. Thus, in the \texttt{DGN-NO-ACT}, the transformation from input to the pre-activations is entirely linear. We call this \textbf{primal linearity}. The disentanglement happens because the ReLU  is completely removed.  

%2. The value network of the DGN is linear in dual `path' variables. We call this \textbf{dual linearity} which stands for the fact that the value network computes path-by-path, and not layer-by-layer. As a result, presenting a $\mathbf{1}$ as input to the value network in \texttt{DGN-NO-ACT} does not degrade performance. The simplifications are : (i) $v_{\Tv}\in \R^{\text{total\,paths}}$ is a vector that does not depend on the input, and (ii) $\phi_{\Tf}(x)\in(0,1)^{\text{total\,paths}}$ is a  simple feature vector. In other words, the value network  learns the paths, and the feature network learns the activations of paths for each input.  While in each layer of the value network GaLUs and the linear operations are entangled, disentanglement happens in the path variables, and we do not have to worry about how learning happens layer-by-layer.

%3. The gates themselves serve the functionality of \emph{lifting} the computations from the primal to the dual, i.e., pre-activations trigger the gates which in turn activate the paths.

%\textbf{Significance.} The salient importance of the \texttt{DGN-NO-ACT} is that it clearly separates the layer-by-layer computations in the feature network and path-by-path computation in the value network. The importance of primal linearity is that we can now use standard linear algebra to `mathematically' interpret the linear transformations from the input to the pre-activations. Also, in the case of specific application domains such as `image classification', these transformations are `filter banks' which have been extensively studied with well known interpretations. The `mathematical' as well as domain specific interpretabilities obviate the need for `locally linear explanation using simpler models': the feature network is entirely linear and is itself simple. The importance of dual linearity is that it gives us a \emph{kernel} based `mathematical' interpretation in the \emph{infinite width regime}. 


%\textbf{DGN-NO-ACT(our model)}(see right diagram in \Cref{fig:dgn}). We replace the ReLUs in the feature network with \emph{identity} maps, i.e., $I(q) = q$. Thus, in the \texttt{DGN-NO-ACT}, the transformation from input to the pre-activations is entirely linear and is amenable to interpertation via standard spectral analysis using linear algebraic tools. The pre-activations trigger the gates, which then dictates the path activity. The value network is given only given $\mathbf{1}$ as input and hence $v_{\Tv}\in \R^{\text{total\,paths}}$ is a vector that does not depend on the input, and $\phi_{\Tf}(x)\in(0,1)^{\text{total\,paths}}$ is a very simple feature vector. % and the output $\hat{y}_{\text{DGN}}(x)=\ip{\phi_{\Tf}(x),v_{\Tv}}=\sum_{p}\phi_\Tf(x,p)v_\Tv(p)$ is equal to \emph{\textbf{the summation of `path value' weighted by the `path activations'}}. 
%Thus, the \texttt{DGN-NO-ACT} can be seen to disentangle the `primal linear' feature network which generates the gates, which in turn activate the paths in the value network which is the `dual linear'.

%\textbf{Remark.} Presenting the value network with $\mathbf{1}$ is very counter intutive, which will get justfied in theory as well as experiments in the next section. As a quick check, we the test accuracies of a DNN $4$ with convolutional layers and global-average-pooling (GAP), its corresponding DGN and \texttt{DGN-NO-ACT} on CIFAR-10 are {\bf{DNN: $80.4\%$,  DGN: $77.4\%$, \texttt{DGN-NO-ACT} : $74.5\%$}}.

%Since $\hat{y}_{\Theta}(x)=\ip{\phi_{x,\Theta},v_{\Theta}}$, during training, as $\Theta$ is learnt, both the NPFs and NPV are also learnt. To understand their roles better, $\phi_{x,\Theta}$ and $v_{\Theta}$ have to be separated.  This is achieved by the deep gated network (DGN) setup (see \Cref{fig:dgn}), which has two networks of \emph{identical architecture} namely the \emph{feature network} ($\Tf\in\R^{d^{\text{f}}_{\text{net}}}$) which holds the NPFs (i.e., the gating information) and the \emph{value network} ($\Tv\in\R^{d^{\text{v}}_{\text{net}}}$) which holds the NPV.  The combined parameterisation is denoted by $\Theta^{\text{DGN}}=(\Tf,\Tv)\in \R^{d^{\text{f}}_{\text{net}}+d^{\text{v}}_{\text{net}}}$.  The feature network is a DNN with ReLUs and the value network is a DNN with \emph{Gated Linear Units (GaLUs)} (terminology used in [\citenum{sss}]) whose output is the product of its pre-activation input $q^{\text{v}}(x)$and the external gating signal $G^{\text{f}}(x)$ (see \Cref{fig:dgn}). In \Cref{fig:dgn}, the main output of the DGN is $\hat{y}_{\text{DGN}}(x)$, while the other output $\hat{y}_{\text{f}}(x)$ is used to \emph{pre-train} the gates (see \Cref{sec:exp}).



==> results.tex <==


\begin{figure*}[t]
\centering
%\begin{minipage}{0.55\columnwidth}
%\centering
%\resizebox{0.99\columnwidth}{!}{
%\input{fig-c4gap-dnn}
%}
%\end{minipage}
\begin{minipage}{0.22\columnwidth}
\centering
\resizebox{0.99\columnwidth}{!}{
\input{fig-dnn-folded}
}
\end{minipage}
\begin{minipage}{0.80\columnwidth}
\centering
\resizebox{0.99\columnwidth}{!}{
\input{fig-dgn-folded}
}
\end{minipage}
\begin{minipage}{0.80\columnwidth}
\centering
\resizebox{0.99\columnwidth}{!}{
\input{fig-dlgn-folded}
}
\end{minipage}
\centering
\resizebox{1.80\columnwidth}{!}{
\begin{tabular}{cccccccc}
\toprule
\multicolumn{8}{c}{Table I}\\
\toprule
Dataset 					& Permute	&C4GAP 				&DGN$(x,x)$ 			&DGN$(x,\mathbf{1})$ 	&DLGN$(x,x)$ 			&DLGN$(x,\mathbf{1})$ 	&$\frac{\text{DLGN}(x,\mathbf{1})}{\text{DNN}}$\\\midrule
\multirow{2}{*}{CIFAR10}		& No			&80.5\tiny{$\pm$0.4} 	&77.4\tiny{$\pm$0.3} 	& 77.5\tiny{$\pm$0.2} 	&75.4\tiny{$\pm$0.3} 	&75.4\tiny{$\pm$0.2}		&$93.66$	\\
						& Yes 		&-- 					&77.3\tiny{$\pm$0.5} 	&77.9\tiny{$\pm$0.6}		&75.9\tiny{$\pm$0.5} 	&76.0\tiny{$\pm$0.5}		&$94.40$	\\\midrule
\multirow{2}{*}{CIFAR100}		& No  		&51.8\tiny{$\pm$0.4} 	&47.4\tiny{$\pm$0.2}		&47.3\tiny{$\pm$0.3} 	&47.4\tiny{$\pm$0.1} 	&48.0\tiny{$\pm$0.2}		&$92.66$\\
						& Yes 		& -- 					&48.4\tiny{$\pm$0.8} 	&49.2\tiny{$\pm$0.9} 	&47.5\tiny{$\pm$1.0} 	&48.4\tiny{$\pm$0.9}		&$93.43$\\
\bottomrule
\end{tabular}
}
\resizebox{1.8\columnwidth}{!}{
\begin{tabular}{cccccccccc}
\toprule
\multicolumn{8}{c}{Table II}\\
\toprule
Dataset 					& Model 		&DNN 				&DGN$(x,x)$ 			&DGN$(x,\mathbf{1})$ 	&DLGN$(x,x)$ 			&DLGN$(x,\mathbf{1})$ 	&$\frac{\text{DLGN}(x,\mathbf{1})}{\text{DNN}}$\\\midrule		
\multirow{2}{*}{CIFAR10}		&VGG16 		&93.6\tiny{$\pm$0.2} 	& 93.0\tiny{$\pm$0.1}  	&93.0\tiny{$\pm$0.1}   	&87.0\tiny{$\pm$0.1}		&87.0\tiny{$\pm$0.2}		&$92.94$	\\
						&ResNet110 	&94.0\tiny{$\pm$0.2} 	& 93.3\tiny{$\pm$0.2} 	&93.2\tiny{$\pm$0.1} 	&87.9\tiny{$\pm$0.2}   	&87.8\tiny{$\pm$0.1} 	&$93.40$	\\\midrule
\multirow{2}{*}{CIFAR100}		&VGG16	 	&73.4\tiny{$\pm$0.3}  	&70.3\tiny{$\pm$0.1} 	&70.5\tiny{$\pm$0.2} 	&61.5\tiny{$\pm$0.2}		&61.5\tiny{$\pm$0.1}		&$\mathbf{83.78}$	\\
						&ResNet110 	&72.7\tiny{$\pm$0.2}		&70.8\tiny{$\pm$0.2} 	&70.8\tiny{$\pm$0.4}		&62.3\tiny{$\pm$0.2} 	&62.7\tiny{$\pm$0.3} 	&$86.24$	\\
\bottomrule
\end{tabular}
}
\caption{\small{Here the gates $G_1, G_2, G_3, G_4$ are generated by the feature network and are permuted as $G_{i_1},G_{i_2},G_{i_3},G_{i_4}$ before applying to the value network. $C_1,C_2,C_3,C_4$ have $128$ filters each. \textbf{Table I and II:} All columns (except the last) show the $\%$ test accuracy on CIFAR-10 and CIFAR-100, and $\%$ of DNN performance recovered by DLGN is in the last column. \textbf{Table I:} For each dataset, the top row has results for vanilla models without permutations (the results are averaged over $5$ runs) and the bottom row has results of $4!-1=23$ permutations (except the identity) for each model (the results are averaged over the $23$ permutations). }}
\label{fig:c4gap-results}
\end{figure*}

\begin{figure*}[t]
\centering
\resizebox{1.8\columnwidth}{!}{
\input{fig-dlgn-sl-folded}
}
\resizebox{1.8\columnwidth}{!}{
\begin{tabular}{ccccccc}
\toprule
\multicolumn{7}{c}{Table III}\\
\toprule
Dataset 			&C1GAP 				&C1GAP-\texttt{16-ENS}		&C1GAP 				&C1GAP-\texttt{16-ENS}		&C4GAP-DLGN-SF	&VGG-16-DLGN-SF\\
\texttt{(epochs)} 		&\texttt{(200)}	 		&\texttt{(200)}			&\texttt{(2000)} 		&\texttt{(2000)}				&\texttt{(50)}					&\texttt{(32)}\\\midrule		
CIFAR-10			&62.2\tiny{$\pm$0.2}		&63.81					&70.0\tiny{$\pm$0.2}		&72.2					&75.1\tiny{$\pm$0.4}				&84.9\tiny{$\pm$0.2}\\ 
CIFAR-100		&36.3\tiny{$\pm$0.2}		&38.23					&42.2\tiny{$\pm$0.3}		&45.47					&47.3\tiny{$\pm$0.6}				&56.3\tiny{$\pm$0.2}\\
\bottomrule
\end{tabular}
}
\caption{\small{C1GAP and C4GAP have width = 512 to make them comparable to VGG-16 whose maximum width is 512. The ensemble size is 16 to match the 16 layers of VGG-16. Note that C4GAP in \Cref{fig:c4gap} has width=128. The last two columns show only DLGN-SF$(x,\mathbf{1})$. We observed the performance of DLGN-SF$(x,x)$ to be $\sim 2\%$ lesser and left it out from Table III for sake brevity. All results except for \texttt{ENS} are averaged over $5$ runs.}}
\label{fig:shallow}
\end{figure*}

